Context-aware Tree-based Deep Model for Recommender Systems

How to predict precise user preference and how to make efficient retrieval from a big corpus are two major challenges of large-scale industrial recommender systems. In tree-based methods, a tree structure T is adopted as index and each item in corpus is attached to a leaf node on T . Then the recommendation problem is converted into a hierarchical retrieval problem solved by a beam search process efficiently. In this paper, we argue that the tree index used to support efficient retrieval in tree-based methods also has rich hierarchical information about the corpus. Furthermore, we propose a novel context-aware tree-based deep model (ConTDM) for recommender systems. In ConTDM, a context-aware user preference prediction model M is designed to utilize both horizontal and vertical contexts on T . Horizontally, a graph convolutional layer is used to enrich the representation of both users and nodes on T with their neighbors. Vertically, a parent fusion layer is designed in M to transmit the user preference representation in higher levels of T to the current level, grasping the essence that tree-based methods are generating the candidate set from coarse to detail during the beam search retrieval. Besides, we argue that the proposed user preference model in ConTDM can be conveniently extended to other tree-based methods for recommender systems. Both experiments on large scale real-world datasets and online A/B test in large scale industrial applications show the significant improvements brought by ConTDM.

==> _w <==
\subsection{Context-aware Tree-based Deep Model}\label{sec:contdm}
%分析现有问题  介绍动机  介绍整体网络结构  
%In TDM, the tree index $\mathcal{T}$ and the user-node preference prediction model $\mathcal{M}$ are closely related with each other.
%Besides,
The sparsity in training data has long been a challenging difficulty in recommeder systems\cite{sarwar2001item}. 
More specifically, the triggered item set in $\{u_i,c_i\}_{i=1}^{N}$ is usually much smaller than the scale of the corpus.
As a result, 
 the quality of the candidate set selected from the entire corpus will be impacted by the inaccurate user-node preference prediction of $\mathcal{M}$ on sparse or even unseen nodes.

%In ConTDM, we 
%To decrease the impact of sparsity and further improve the recommendation accuracy, we propose a context-aware tree-based deep model in this section.
%In ConTDM,  
In this section, we introduce the proposed framework of context-aware tree-based deep model.% which framework is shown in Fig \ref{fig:ConTdm}.
%In ConTDM, both the training and retriveal process
% 需要一个更自然和高级以及前后照应的过渡
%To decrease the impact of sparsity and further improve the recommendation accuracy, a novel user preference model is proposed in ConTDM.
Given a user $u$ and a current node $n$ to be predicted by the user preference model. 
The main idea of ConTDM is utilizing the useful contexts between nodes of $\mathcal{T}$ in predicting $n$ to decrease the impact of sparsity and further improve the recommendation accuracy.
To achieve this, a novel user preference model is proposed in ConTDM.
Besides, the training and retriveal of ConTDM on a binaray tree index follows the process of TDM introduced in Section \ref{sec:tdm}. 
The framework of ConTDM is shown in Fig \ref{fig:ConTdm}.

As shown in Fig \ref{fig:ConTdm}(a), the user feature used in the proposed user-node preference prediction model is a combination of hierarchical user behavior sequences\cite{zhu2019joint} and other useful features such as user profile.
Denoting $(c_1,c_2\cdots c_n)$ as the historical behavior sequence of the user $u$, the hierarchical user feature is represented as $(b_j(c_1),b_j(c_2)\cdots b_j(c_n))$ when the current node in prediction is in level $l$.

Firstly, all node embeddings contained in the hierarchical user feature and the target node are put into a graph convolutional layer to get graph embeddings containing neighbour contexts.
To include more historical behaviors for each user without much increasing the computation at the same time, 
 historical behaviors are divided into different time windows and the graph embeddings of the hierarchical user feature in the same time window are averaged.
After fusing the averaged graph embedding in each time window with the target graph embedding through an attention unit,
all the hierarchical user embeddings, other user embeddings and the target embedding is concatenated as the input of the next several fully connected layers with pReLu activation function.  


 
%Then the embeddings 
%the proposed user-node preference prediction model takes the hierarchical user behavior sequences\cite{} and other 

%In this section, we introduce the contex-aware user preference prediction model $\mathcal{M}_{con}$ used in ConTDM.
%Both training and retriveal process follows TDM.

%Contexts between nodes are imported in $\mathcal{M}_{Con}$ to remit the impact of sparsity.
%The structure of $\mathcal{M}_{con}$ is shown in Fig \ref{fig:ConTdm}.
%To conquer this issue, we further study the interdependence between $\mathcal{T}$ and $\mathcal{M}$. Contexts 

%In ConTDM, we follow the framework of TDM in training and retriveal. 

%For large scale recommeder system, the training data is usually very sparse and largely add the difficulty of training the user preference model, which means the behaved items are only a small proportion of the corpus. On the other hand, brutely adding more training data from more days will linearly adding the training time cost. 

%To conqure this issue without losing much effiency, we propose the user preference model used in ConTDM in this subsection.  In ConTDM, we sovle the sparsity problem by better utilizing the context information brought by the tree index and user behavior sequences. Our main observation is that importing related nodes or items is helpful for current  prediction.

%In ConTDM

%The structure of the proposed context-aware user preference model $\mathcal{M}$ is shown in Fig \ref{fig:ConTdm}. For convenience, we only take the hierarchical user behavior sequence proposed in JTM as the user feature. The other features such as user profile can be used directly in ConTDM. 

%Compared with deep interest network used in TDM, there are two main improvements in the design of $\mathcal{M}$: 1) The user preference presentation on the parents' nodes are passed to the current layer as the input of the parent context fusion layer. 2) A graph embedding layer merging information from neighbour nodes is used. 

%iThe effect of These two fusion layer is explained in the next two subsections. 


\subsubsection{Parent Fusion Layer}

Denote $v(n_l)$ as the PReLu's output of $\mathcal{M}$ for node $n_l$ in $l_{th}$ level of the tree index. In DIN, the last sofmax layer takes $v(n_l)$ as the input to predict the user preference probability. In this paper, we take it as user node preference representation.

For node $n_l$, the parent fusion layer takes $v(n_l)$ and $v(pa(n_l))$ as input where $pa(n)$ returns the parent node of $n$. Then it returns the fused user node preference representation after passing an attention unit. 

Our main motivation is to use the context contained in $v(pa(n_l))$ to assist the prediction for $n_l$. This brings two main benefits:

\begin{itemize}
    \item Explainability. In TDM, each node is an abstraction of its children. Furthermore, with hierarchical user feature, $v(n_l)$ is an effective abstract user node preference representation for node $n$ in the $(l-1)_th$ level. The parent fusion layer graps the essence that the retriveal of TDM is to make prediction from coarse to detail. Intuitively, it is helpful to import $v(pa(n_l))$ in the prediction of $\hat p(n_l\vert u)$. 
    \item Non-sparsity. In higher levels, the task of $\mathcal{M}$ is to make user preference prediction of node $N$ with hierarchical use features, which is also an abstraction of the raw user feature with nodes in higher levels. Noticing that the number of nodes in higher levels is much smaller, both the sparsity of training samples in higher levels and prediction difficulty is largely decreased. An obvious example is that the recall in higher levels is usually very high for higher levels. Therefore, it is benefitial to weaken the impact of sparsity in lower levels. 
    \item Effiency. With the beam search process from top to down, $v(n_l)$ can be passed and reused. The total increase of computation is the attention unit which is very little compared with total computation. Besides, the parent fusion layer can be cascaded to further improve the performance if needed. 
\end{itemize}

\subsubsection{Graph Converlution Layer}

Graph-based methods have been widely used to solve sparsity problems recently. In ConTDM, we design a non-parameterized graph embedding unit considering the efficiency. Other popular methods such as GraphSage, GCN, GAT can also be used. For node $n$, the graph embedding unit firstly average the embeddings of its neighbours and then concat with $n's$ embedding to import neigbhour context and highlight the role of $n$ at the same time.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/Graph.eps}
\caption{Graph}\label{fig:Graph}
\end{figure}

Obviously, the reasonability of the graph used in the graph embedding layer matters. The method proposed in () is used to construct the subgraph of leaf level.  
However, in ConTDM, a hierarchical graph is needed. Inspired by hierarchical user features, the raw user behavior can be traced up to each levels to work as the extracted user behavior to the corresponding level. Then the subgraph in each level can be contructed as the leaf level. 

The construction process of graph is show in Fig \ref{fig:Graph}. The main idea is that there should be an edge if a co-occurrence pair of items. For each raw user behavior sequence, we first trace up it to all the levels and count all the co-occurrence pairs that the time stamp gap is smaller than a limit value. Then a new edge is added if there is originally no edges between paris and the weights increase otherwise. Finally, the number of neighbours for each node is truncated up to a limit number by the weights to avoid the number of neighbours is too big.

With the graph embedding layer, the representation of a item can be enriched by its neighbours and the sparsity is sovled. Furthermore, more sequences can be used in the construction of graph than the training samples and further improve the effiency.


==> section3_2.tex <==
\subsection{ConTDM on Multipath Tree}\label{sec:contdm-mul}

The max-heap like property shown in Eq (\ref{eq:heap}) is the footstone of Tree-based Deep Model. 
According to Eq (\ref{eq:heap}), the estimated user node preference probability $\hat p(b_j(c)\vert u)$ given a positive training sample $(u,c)$ should be maximized among nodes in corresponding layer for any $j$. 
%the sucess of TDM to achive the item that the user most prefers from the total corpus. 
%To approximate the property for each user to the maximize degree, the joint probability along the path to the root node from the positive leaf node is maximized, as show in eq(to fill). 
%However, because of the limitation of the deep model's capcity, the max-heap like property can only be guranteed for  each node in the sense of average. It can hardly be satisfied especially for those nodes that cotain user set with large variance.
%By building a more proper binaray tree index, this problem can be partially solved and the training loss can be further optimized. However, the users contained by a node cannot be further adjusted because  the path to the root node from a leaf node is fixed with a binary tree index.  
 However, this property can hardly be satisfied for each training user or even unseen user because the user node preference model can not be perfectly trained. 
Actually, given a trained user preference model $\mathcal{M}$, 
%and a user who prefers item $\mathcal{c}$, the best path from $c$ to the root node may not be the fixed one decided by the binaray tree index. 
%However, 
there could be another node $n$ in level $l$ making that $\hat p(n\vert u) > \hat p(b_l(c)\vert u)$,
which leads the beam search retrieval to get suboptimal leaf results.
In this situation, $b_{l+1}(c)$ should be a child of $n$ for user $u$ to make Eq(\ref{eq:heap}) satisfied
and retrieve the most preferred item.
%which means the path should contains $n$ otherthan $b_l(c)$.
In other words, an extra edge between $n$ and $b_{l+1}(c)$ should be added to make the tree index from binary to multipath.
%As a main benefit, the best path  
However, this also brings two problems:
\begin{itemize}
    \item If we want to find a better path on $\mathcal{T}$ for each user to train $\mathcal{M}$ under the loss in Eq (\ref{loss}), 
        traversing all possible paths on a fully connected multipath tree index is computationally unacceptable.  
        %For the full connection multi-way tree, the computation for a single user to find the best path is exponentially explosed. 
        Some restrictions on the structure of $\mathcal{T}$ and a proper search strategy are necessary.   
    \item  %In the process of beam search in TDM, all the children of the top scored nodes are put into the next beam to make prediction. If the same value of top k is used in beam search, the overall number of nodes scored also increases. If a smaller $k$ is used for multi-way tree index, the generalization ability may be restricted too.
        The total number of predicted nodes in retrieval for each user increases linearly with the average branches of $\mathcal{T}$ according to the beam search strategy.
        To conquer this issue, an accelerated model is needed. 
\end{itemize}

 According to discussions above, we extend ConTDM to the more challenging multipath tree index in this section.
 With the constructed graph and an upgraded context-aware user preference prediction model, we will show in the following two subsections that both problems above can be effectively solved.
% Firstly, The graph-based multi-way tree index and the simplified user preference prediction model are introduced in Section \ref{sec:multi-tree}. 
% Then the new framework of ConTDM on multi-way tree index is shown in Section \ref{sec:new-framework}.
%We firstly show the multi-way tree and the simplified user preference prediction model used to conquer the problems above. i
%Then we give the whole process to train ConTDM for multi-way tree index. 

\subsubsection{Multipath Tree Index and User Preference Model} \label{sec:multi-tree}

Firstly, we build the multipath tree index based on the binary tree index and the constructed graph, as shown in Fig \ref{fig:Graph}(c).  
%With the constructed graph and a binary tree index, we can naturally extend the binaray tree index to a multi-way tree index as shown in Fig \ref{fig:Graph}. Compared with the full connection multi-way tree index, 
For each node $n$, we add extra edges between $n's$ parent and $n's$ neighbours.
Besides, a greedy pruning by weights is made to avoid a node having too many possible parents.
%Besides, we only keep no more than $m$ children by weights for each node to avoid that it has too many children and hence contains too many users. Then, we also avoid $n$ to be a parent node for too many nodes by pruning. 
  Considering that neighbours are similar nodes constructed by the most frequent co-occurrence pairs, the variance of possible paths on the graph-based multipath tree index for each item will be effectively controlled.  
  %, which benefits the training of $\mathcal{M}$.% and also motivates the generalization ability. 
  %Besides, the neighbours of nodes in the current candidate set are a good supplement among other nodes in retrieval, because   
%In the construction of graph, we select items most frequently co-occured as the neighbours, which means their similarity is usually high. Besides, the graph embedding layer usually makes the score of $n$ close with its neighbours. If the current model $M$ is well leaned, the quality of positive $n$ should be good (although not the best maybe). Then its neighbours should be a good subset of all nodes in this level to find a better path.
%\subsubsection{Simplified User Preference Model} \label{sec:simp-model}

%On the other hand, a simplified user preference model is used to avoid the linearly increase of computation in retrieval.
%  \textcolor{blue}{
As explained in Section \ref{sec:mtl-layer}, the parent user node preference representation $v(pa(n))$ is a useful auxiliary feature in user preference prediction. % estimating $\hat p(n_l\vert u)$.
Inspired by this, we modify the parent fusion layer with an extra fusion unit to get the multipath parent fusion layer used in the context-aware user preference model for multipath tree index, as shown in Fig \ref{fig:ConTdm}(b). 
More exactly, the fused user preference representation on the current node $n$ is computed by
\begin{equation}
    {\tilde{v}}_f(n) = PReLU\left(W* Concat\left(h(n),h(n)\odot v_f(pa(n)),v_f(pa(n))\right)+b\right),
\end{equation}
where $h(n)$ is the embedding of $n$, $v_f(pa(n))$ is the fused user preference representation on the parent of $n$ computed by Eq (\ref{eq:fuseunit}).
Instead of fusing $v(n)$ and $v(pa(n))$ , we use the fusion of $h(n)$ and $v_f(pa(n))$ in estimating $\hat p(n\vert u)$.
Essentially, we are directly using the coarse user preference representation achieved in higher levels to predict $n$. 
To further improve its capacity, we use  $v_f(pa(n))$ to import two layers of vertical contexts.
%In the simplified user preference model, the parent fusion layer directly use $v(pa(n_l))$ and the embedding of $n_l$ as input in estimating $\hat p(n_l\vert u)$, as shown in Fig \ref{fig:ConTdm}.
As a main benefit, $v_f(pa(n))$ can be reused for all children of $pa(n)$ on the multipath tree index to largely reduce the total computation in beam search retrieval. %}
%\footnote{
A more careful analysis about the computation complexity is provided in Appendix \ref{appendix:computation}. %\ref{appendix:computation}.
%Since vertical contexts $v_f(pa(n))$

%In ConTDM, we design a parent fusion layer to import the parent user node preference representation to assist the current node's prediction. Our starting point is that the abstract $v_{l-1}(n)$ also has the ability to classify $n$ in level $l$. 
%To control the extra computation brought by the multi-way tree index, we design a simplified parent fusion layer shown in Fig\ref{fig:ConTdm}. Instead of using  $v_l(n)$ and $v_{l-1}(n)$, we directly put $v_{l-1}(n)$ and $emb(n)$ to the attention unit in classification. 
%As the main benefit, for node $n$ and its parent $pa(n)$ and given $p(n)$, which computation complexity equals to that in ConTDM, the extra computation complexity for each brother is only an extra attention unit as $v_{l-1}(n)$ can be reused. The extra computation is usually less than $10\%$.

\subsubsection{Algorithm}\label{sec:new-framework}

With the graph-based multipath tree index $\mathcal{T}$ and the modified context-aware user preference model $\mathcal{M}$. We are ready to introduce the new training framework of ConTDM on multipath tree index, as shown in Algorithm \ref{alg:ConTdm}.  

\begin{algorithm}[t]
\caption{Training framework of ConTDM on multipath tree index}\label{alg:ConTdm}
\begin{algorithmic}[1]
    \REQUIRE Initial user preference model $\mathcal{M}$, initial binary tree $\mathcal{T}_b$, graph $\mathcal{G}$, training data $\{(u_i,c_i)\}_{i=1}^N$.
    \STATE Construct the multi-way tree index $\mathcal{T}$ with $\mathcal{T}_b$ and $\mathcal{G}$.
    \STATE Greedily generate the best path to the root node for each $(u_i,c_i)$.
    \STATE Finetune $\mathcal{M}$ with the generated paths under loss in Eq (\ref{loss}).
%\ENDFOR
\ENSURE Finetuned model $\mathcal{M}$ and multipath tree index $\mathcal{T}$.
\end{algorithmic}
\end{algorithm}

%\textcolor{blue}{
The input of ConTDM on multipath tree index is a pretrained model $\mathcal{M}$ on the binary tree index $\mathcal{T}_b$ and the graph $\mathcal{G}$. We firstly build a multipath tree index as explained in the last subsection. For each training sample $(u_i,c_i)$, we can greedily generate a new path from $c_i$ to the root node on $\mathcal{T}$. 
For example, among all $c_i's$ parent nodes on $\mathcal{T}$, we choose the one with the biggest $\hat p(n\vert u)$ estimated by the pretrained model $\mathcal{M}$ as the user specific parent in finetuning $\mathcal{M}$. 
This process repeats until the root node is arrived.
Besides, the most frequent path for each item in the leaf level is used to generate the hierarchical user behaviors. The hierarchical features are used as the input feature of ConTDM.
%to promote the max-heap like property in Eq (\ref{eq:heap}). 
%the best parent from all the possible parents with the largest score from down to top.
%Generally, the total training loss will all be smaller.i
Finally we finetune $\mathcal{M}$ with the selected paths.
In retrieval, the beam search process is also used.%}

%Besides, steps 2-3 can be repeated to further improve the recommendation accuracy. 

%While training, the hierarchical user feature keep unchanged as the binary tree. Steps 2-3 can also be repeated if needed. 

%To conquer the impact of 'average user', a multi-way tree index is prefered.
%In prior of the classification ability of abstract user preference representation and the similarity between node and its neighbours, ConTDM with a simplified parent fusion layer can be used in a multi-way tree index without much increase of computation in a single retrieval. Besides, the simplified parent fusion layer can also release the capcity to adopt more complex deep model with the same overall complexity to achive better preformance if needed, as will be shown in the experiment section.


==> section4.tex <==
\section{ConTDM on Multi-way Tree}\label{section:method2}
With children selection mechanisim, we can extend ConTDM to multi-way tree index, which includes binary tree as a special case. (To be decide how to write)  


